Meta-learning with implicit gradients in a few-shot setting for medical image segmentation

Widely used traditional supervised deep learning methods require a large number of training samples but often fail to generalize on unseen datasets. Therefore, a more general application of any trained model is quite limited for medical imaging for clinical practice. Using separately trained models for each unique lesion category or a unique patient population will require sufficiently large curated datasets, which is not practical to use in a real-world clinical set-up. Few-shot learning approaches can not only minimize the need for an enormous number of reliable ground truth labels that are labour-intensive and expensive but can also be used to model on a dataset coming from a new population. To this end, we propose to exploit an optimization-based implicit model agnostic meta-learning (iMAML) algorithm under few-shot settings for medical image segmentation. Our approach can leverage the learned weights from diverse but small training samples to perform analysis on unseen datasets with high accuracy. We show that, unlike classical few-shot learning approaches, our method improves generalization capability. To our knowledge, this is the first work that exploits iMAML for medical image segmentation and explores the strength of the model on scenarios such as meta-training on unique and mixed instances of lesion datasets. Our quantitative results on publicly available skin and polyp datasets show that the proposed method outperforms the naive supervised baseline model and two recent few-shot segmentation approaches by large margins. In addition, our iMAML approach shows an improvement of 2%-4% in dice score compared to its counterpart MAML for most experiments.

==> takeout.tex <==
%% MSC codes here, in the form: \MSC code \sep code
%% or \MSC[2008] code \sep code (2000 is the default)
%\MSC 41A05\sep 41A10\sep 65D05\sep 65D17
%% Keywords

% \KWD Gastrointestinal endoscopy challenges\sep Artificial Intelligence
% \sep Medico Task 2017 \sep Medico Task 2018 \sep Kvasir \sep Nerthus \sep BioMedia 2019 Grand Challenge \sep Health informatics

%There has been significant progress made in the ain the application of \ac{DL}-based methods for the semantic segmentation of clinically relevant anomalies in the field of medical imaging~\citep{horng2017creating,brown2018automated,hinton2018deep}.

%Thus, for quick and better optimization during meta-learning, we use the \ac{iMAML} algorithm~\citep{rajeswaran2019meta}. 
% Needs rewriting!!! TODO

%%%%
% TODO: brief overview of what are component
% Brief on what is new here?
%%%

%TODO:
% 0) Define support and query; meta-training and meta-testing events
% Continual learning: remembering new tasks without forgeting old tasks
% 1) Define tasks 
% 2) define shots
% DUE TO IMAGES HAVING THESE DATASETS!!!



%% Strength: improve++àment in results due to your approach!!!
% Recall the result and discuss - cat I (why important and what other ) - tab 2 - conclude what it shows and how it improves your performance 
%
% cat II (why it is important, have someone done, gap and what your results say - performance improvement of method) - tab ? - conclude;
% cat III (why it is important, have someone done, gap and what your results say - performance improvement of method) - tab ? - conclude; cat III - conclusion 
% Strength of the method pointing figure 2 and -- representations learnt in Fig 3 & 4 -- why visual maps and how it demonstrate strength of algorithm- 
%
% Paragraph- suggestions (hypothesis)
%



%Segmentation of region-of-interest in medical images is important for quantification of disease progression and treatment.

%Missing a connection from what you say before to the image segmentation problem, Maybe you mean especially medical image segmentation algorithms require a lot of diverse and accurate data if they are intended to be generalizable

% TODO --> include figure: sub-optimal results (images with DSC < 60 %) 2 for skin, 2 for Kvasir and 2 for capsule (material to discuss!!!)

where data is scarce for a particular disease and/or multi-modal data scenario for training ML model.


where multi-modal datasets are available or scarcity of dataset for a particular disease or findings. 

This meta-learning approach can potentially contribute to the development of a clinical systems for real-world application where multi-modal dataset  can be scarce for a particular disease or findings.

%Figure~\ref{fig:base_activation} shows the activation map from the 17th convolutional layer of the baseline model. Similarly, Figure~\ref{fig:base_meta} shows the activation map from the 17th layer of our meta-learned model.
